Orthogonalized SGD and Nested Architectures for Anytime Neural Networks

We propose a novel variant of SGD customized for training network architectures that support anytime behavior: such networks produce a series of increasingly accurate outputs over time. Efficient architectural designs for these networks focus on re-using internal state; subnetworks must produce representations relevant for both immediate prediction as well as refinement by subsequent network stages. We consider traditional branched networks as well as a new class of recursively nested networks. Our new optimizer, Orthogonalized SGD, dynamically re-balances task-specific gradients when training a multitask network. In the context of anytime architectures, this optimizer projects gradients from later outputs onto a parameter subspace that does not interfere with those from earlier outputs. Experiments demonstrate that training with Orthogonalized SGD significantly improves generalization accuracy of anytime networks.

==> Makefile <==
# programs
LATEXMK  = latexmk
PDFLATEX = pdflatex -halt-on-error -interaction=nonstopmode
TOUCH    = touch
RM       = rm

# compilation targets
targets   := main
pdf_files := $(addsuffix .pdf,$(targets))

# intermediate files
d_files   := $(wildcard $(addsuffix .d,$(targets)))
aux_files := $(addsuffix .aux,$(targets))
bbl_files := $(addsuffix .bbl,$(targets))
blg_files := $(addsuffix .blg,$(targets))
brf_files := $(addsuffix .brf,$(targets))
log_files := $(addsuffix .log,$(targets))
fls_files := $(addsuffix .fls,$(targets))
fdb_files := $(addsuffix .fdb_latexmk,$(targets))
out_files := $(addsuffix .out,$(targets))

# default target
.PHONY: default
default: all

# all targets
.PHONY: all
all: $(pdf_files)

# build rules
$(pdf_files): %.pdf: %.tex
	@$(LATEXMK) -pdf -pdflatex="$(PDFLATEX)" -M -MF $*.d $*.tex;\
	 $(TOUCH) $*.pdf $*.d
ifneq ($(d_files),)
-include $(d_files)
endif

# clean
.PHONY: clean
clean:
	$(RM) -f\
            $(aux_files)\
            $(bbl_files)\
            $(blg_files)\
            $(brf_files)\
            $(log_files)\
            $(fls_files)\
            $(fdb_files)\
            $(out_files)\
            $(d_files)\
            $(pdf_files)

